AutoQNN: An End-to-End Framework for Automatically Quantizing Neural Networks

Exploring the expected quantizing scheme with suitable mixed-precision policy is the key point to compress deep neural networks (DNNs) in high efficiency and accuracy. This exploration implies heavy workloads for domain experts, and an automatic compression method is needed. However, the huge search space of the automatic method introduces plenty of computing budgets that make the automatic process challenging to be applied in real scenarios. In this paper, we propose an end-to-end framework named AutoQNN, for automatically quantizing different layers utilizing different schemes and bitwidths without any human labor. AutoQNN can seek desirable quantizing schemes and mixed-precision policies for mainstream DNN models efficiently by involving three techniques: quantizing scheme search (QSS), quantizing precision learning (QPL), and quantized architecture generation (QAG). QSS introduces five quantizing schemes and defines three new schemes as a candidate set for scheme search, and then uses the differentiable neural architecture search (DNAS) algorithm to seek the layer- or model-desired scheme from the set. QPL is the first method to learn mixed-precision policies by reparameterizing the bitwidths of quantizing schemes, to the best of our knowledge. QPL optimizes both classification loss and precision loss of DNNs efficiently and obtains the relatively optimal mixed-precision model within limited model size and memory footprint. QAG is designed to convert arbitrary architectures into corresponding quantized ones without manual intervention, to facilitate end-to-end neural network quantization. We have implemented AutoQNN and integrated it into Keras. Extensive experiments demonstrate that AutoQNN can consistently outperform state-of-the-art quantization.

==> sections/05-02-SalientObjectDetection.tex <==
\input{tables/sod_results}
\cumparagraph{Salient Object Detection}

We employ MSRA-10K~\cite{MSRA10K} as the training set, and take MSRA-B~\cite{msra}, DUTs~\cite{duts}, and DUT-OMRON~\cite{duts} as the validation set.
All the images in these datasets are resized to $224\times 224$ for the training and test.
Three models including UNet~\cite{ronneberger2015unet}, LinkNet~\cite{chaurasia2017linknet}, and FPN~\cite{lin2017fpn} are involved in the evaluation.
We take ResNet50~\cite{he2016resnet} as the backbone network for these models and the implementation details can be found here\footnote{https://github.com/qubvel/segmentation\_models, \text{Oct. 2022}.\label{segementation_model_note}}.
Besides, we take the intersection over union (IoU), F$_1$-measure (F$_1$), E-measure (EM)~\cite{fan2018enhanced}, and mean absolute error (MAE) as the evaluation metrics.
The implementations of IoU, F$_1$ and MAE can be found here\textsuperscript{\ref{segementation_model_note}}, and EM refers to \cite{fan2018enhanced}.
We employ ClipQ for model quantization and do not quantize the first and last layers of models.
\gcc{We set the average bitwidth as $2$ for QPL to apply an extremely low-bitwidth quantization for these large SOD models for great computing benefits.}

The quantitative comparison results are in \tabref{tab:comparing_results_on_sod}. 
The model size and memory footprint of UNet are reduced by \text{14.88}$\times$ and \text{172.56}$\times$, respectively, when it is quantized into the average bitwidths of 2.15/2.76 with AutoQNN, and the performance degradation in four metrics across all datasets is less than \text{0.01}. 
AutoQNN also shrinks the memory footprint of FPN and LinkNet by \text{155.67}$\times$ and \text{172.64}$\times$ through quantizing models from full precision into low precision with average bitwidths of 2.20/2.99 and 2.20/2.65, respectively, and only incurs slight performance degradation which is not more than \text{0.018} in all metrics across three datasets.
The results demonstrate that QPL can reduce memory footprint by using the extremely low-bitwidth weight and activation with negligible performance degradation. 
This highlights that QPL can search for a suitable quantizing strategy to maintain comparable feature extraction quality of SOD models. 




==> sections/07-Acknowledge.tex <==
% \section{\gcc{Acknowledgment}}
{\bf \gcc{Acknowledgements}}
\gcc{This work is partially supported by the National Key Research and Development Program of China (2018YFB2100300), 
the National Natural Science Foundation (62002175), 
the Natural Science Foundation of Tianjin (19JCQNJC00600),
the State Key Laboratory of Computer Architecture (ICT,CAS) under Grant No. CARCHB202016,  
and the Innovation Fund of Chinese Universities Industry-University-Research (2020HYA01003).}

==> tables/cadidate_schemes.tex <==
\renewcommand{\arraystretch}{1.1}
\begin{table*}[!ht]
    \centering
    \caption{The candidate quantization schemes and the \sArt~works.}
    \label{tab:quantization_schemes}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{c|c|l|c}\Xhline{1.5pt}
        Bitwidth & Names & Implementations & Comparison works \\\Xhline{1.5pt}
        \multirow{1}{*}{1} & Binary (B) & $d_q=E(|d_f|)\cdot sign(d_f)$ & BC~\cite{Binaryconnect}\\\Xhline{0.5pt}
        \multirow{2}{*}{2}& \multirow{2}{*}{Ternary(T)} & $d_q=\alpha\cdot C(R(d_q/\beta),-1,1)$ & TNN~\cite{alemdar2017ternary}, TC~\cite{Ternaryconnect}\\
        &&$~~~~s.t.~\alpha=E(|d_f(i)|), i\in\{i||d_f(i)|>0.7E(|d_f|)\}, \beta=1.4\cdot E(|d_f|)$~\cite{TWNs}&\\\Xhline{0.5pt}
        \multirow{2}{*}{2} & \multirow{2}{*}{Quaternary (Q)} & $d_q=\alpha\cdot C(R(d_q/\beta-0.5),-2,1)+0.5$& $\mu$L2Q~\cite{cheng2019uL2Q}, VecQ~\cite{VecQ} \\
        &&$~~~~s.t.~\alpha$ and $\beta$ refer to \cite{VecQ} &\\\Xhline{0.5pt}
        \multirow{2}{*}{2-8} & FixedQ (F) & $d_q= 2^p\cdot R(d_f/2^p)$ & FP~\cite{gysel2016hardware}\\
        &&$~~~~s.t.~p=\lfloor\log_2(\max(|d_f|))\rfloor-(k-2)$&\\\Xhline{0.5pt}
        \multirow{2}{*}{2-8} & ZoomQ (Z) & $d_q=\alpha\cdot R(d_f/\alpha)$ & Dorefa-Net~\cite{DSQ}\\
        &&$~~~~s.t.~\alpha=\max(|d_f|)/(2^{k-1}-1)$&\\\Xhline{0.5pt}
        \multirow{2}{*}{2-8} & LinearQ (L) & $d_q=\alpha\cdot C(R(d_f/\alpha),-2^{k-1}+1,2^{k-1}-1)$ & DSQ~\cite{DSQ}, QIL~\cite{QIL}\\
        &&$~~~~s.t.~\alpha=3\sigma_{d_f}/(2^{k-1}-1)$&\\\Xhline{0.5pt}
        \multirow{2}{*}{2-4} & \multirow{2}{*}{PotQ (P)}&$d_q=\alpha\cdot H(d_f/\alpha)$ & ENN~\cite{ENN2017}, INQ~\cite{INQ2017}\\
         & &$~~~~s.t.~H:\mathbb{R}^{|d_f|}\rightarrow\mathbb{Q}^{|d_q|},\mathbb{Q}=\{0,\pm 2^0,\pm 2^1,\cdots, \pm 2^{2^{k-1}-2}\}$, $\alpha$ refers to \cite{ENN2017} &\\\Xhline{0.5pt}
        \multirow{3}{*}{2-8}& \multirow{3}{*}{ResQ (R)} & $d_q=\sum_{i=1}^{k}(E(|v_i|)\cdot sign(v_i))$ & ABC-Net~\cite{ABC-Net}, LQ-Nets~\cite{LQ-Nets} \\
        &&$~~~~s.t.~v_i=\begin{cases}
        d_f,~i=1\\
        d_f-\sum_{j=1}^{i-1}(E(|v_j|)\cdot sign(v_j)),~i>1
        \end{cases}$&\\
        \Xhline{1.5pt}
    \end{tabular}
\end{table*}
